DisenPOI: Disentangling Sequential and Geographical Influence for Point-of-Interest Recommendation

Point-of-Interest (POI) recommendation plays a vital role in various location-aware services. It has been observed that POI recommendation is driven by both sequential and geographical influences. However, since there is no annotated label of the dominant influence during recommendation, existing methods tend to entangle these two influences, which may lead to sub-optimal recommendation performance and poor interpretability. In this paper, we address the above challenge by proposing DisenPOI, a novel Disentangled dual-graph framework for POI recommendation, which jointly utilizes sequential and geographical relationships on two separate graphs and disentangles the two influences with self-supervision. The key novelty of our model compared with existing approaches is to extract disentangled representations of both sequential and geographical influences with contrastive learning. To be specific, we construct a geographical graph and a sequential graph based on the check-in sequence of a user. We tailor their propagation schemes to become sequence-/geo-aware to better capture the corresponding influences. Preference proxies are extracted from check-in sequence as pseudo labels for the two influences, which supervise the disentanglement via a contrastive loss. Extensive experiments on three datasets demonstrate the superiority of the proposed model.

==> intro_temp.tex <==
\section{Introduction}
The rapid growth of Location-Based Social Networks (LBSN), have facilitated the development of Point-of-Interest (POI) recommendation, which lies at the heart of various location-based services, including location-based advertising and online food-delivery. And it serve as the backbone for numerous popular Apps, such as Foursquare, Gowalla and Meituan. A POI can be a restaurant, a hotel, a scenic spot, or any location-tagged item. Location information is much more than an ordinary feature dimension in POI recommendation: it builds up a network structure among POIs, inter-connected by both their interactive history sequence and geographical affinity. 

% The Point-of-Interest (POI) lies at the heart of location-based services (LBS), serving as the backbone for numerous popular Apps, including Foursquare, Gowalla and Meituan. It is the basis of various down-stream tasks, including location-based advertising and online food-delivery services. A POI can be a restaurant, a hotel, a scenic spot, or any location-tagged item. Location information is much more than an ordinary feature dimension in POI recommendation: it builds up a network structure among users and POIs, inter-connected by both their interactive history sequence and geographical affinity. 
%This social structure can be effectively expressed using graph structure. As is shown in Figure \ref{fig:model_1}, a user's visit to POI $v_i$ can be induced by disentangled influences from its neighboring nodes in the geographical graph and the sequential graph. The disentangled influences can be neatly modeled using two separate graph neural networks (GNNs).

\begin{figure}[t]
    \centering
    
    \includegraphics[width=\linewidth]{Figs/model_fig1v2.pdf}
    
    \caption{An illustration of disentangled influences behind check-ins. A visit to $v_4$ is influenced by its neighbouring nodes from geographical and sequential graph.}
    \label{fig:model_1}
\end{figure}

Recent works on POI recommendation endeavor to integrate geographical influences with sequential transitions of the check-in data. Sequence-based methods like LSTPM ~\cite{sun2020go} combines user's long-term interest with geo-dilated short-term interest, using geographical affinity as an auxiliary in modeling sequence behavior. GeoIE ~\cite{wang2018exploiting} explicitly uses physical distance to model user-specific geographical influence, and GTAG ~\cite{sun2014graph-based} performs preference propagation based on physical distance and time-slot affinity. Despite the versatility of these sequential POI recommenders, most existing approaches lack the ability to explicitly uncover the collaborative signals. Since graph-structured commonly exist in interactions, as well as between POIs of check in data, a promising approach is to leverage the rich graph structure to exploit high-order connectivity between POIs.
%Since these check in data locates in the Euclidean space, one promising approach to exploit high-order connectivity is to leverage graph structure.

% a notable limitation is they lack explicitly modeling the POI relationships

Inspired by the great success of graph neural networks (GNNS), GNNs have been extensively used for recommendation for their strong capability of capturing similarity between high-order neighbours. According to different graph topology structure, prevalent modeling schemes thus can be categorized into two types. The first type is CF-based, which collects the collaborative signal on the user-POI bipartite graph, e.g. NGCF ~\cite{wang2019neural} and LightGCN ~\cite{he2020lightgcn}. The second type is sequence-based, which propagates along the user’s interactive sequence graph with POIs, e.g. SR-GNN ~\cite{wu2019session}. Although these paradigms provide valuable insight as to organizing interaction data into graph structure for POI recommendation, they do not leverage geographical relationship, which is a prominent characteristic in POI recommendation.
%However, these approaches do not leverage sequential influence and geographical influence in a bi-lateral way. Ideally, sequential influence and geographical influence should be regarded as equal counterparts. As long as one influence is dominant in the model architecture, yet the other serves only as auxiliary signal, the results learned by the model would always be biased towards only one of the influences. 

%GNNs have been extensively used to alleviate data sparsity and cold-start issues for click-through rate (CTR) prediction and personalized recommendation, which represents users and POIs as graph nodes. Prevalent modeling schemes can be categorized into two types. The first type is CF-based, which collects the collaborative signal on the user-POI bipartite graph, e.g. NGCF ~\cite{wang2019neural} and LightGCN ~\cite{he2020lightgcn}. The second type is sequence-based, which propagates along the user’s interactive sequence graph with POIs, e.g. SR-GNN ~\cite{wu2019session}. Although these paradigms provide valuable insight as to effectively organizing graph data in POI recommendation, they fail to adequately incorporate location relationship and model geographical influences. 

In fact, sequential influence and geographical influence should be regarded as equal counterparts, which are two of the major driving forces in POI recommendation. As the toy example in Figure \ref{fig:model_1} shows, a user's visit to $v_4$ is influenced by its neighbouring nodes from geographical and sequential graph. On the one hand, users are apt to re-visit familiar POIs that have showed up in their interaction sequence. For example, frequent visits to clothing stores may reveal a user's preference in fashion, which indicates that a similar clothing store has more chance to be the next-to-visit POI. On the other hand, POIs in the vicinity are also more likely to be visited. For instance, a user just came out of a shopping mall in downtown is more likely to visit a fast food shop nearby for lunch, instead of his/her favourite restaurant in the countryside. However, user preferences learned in previous POI recommendation approaches always entangled with each other, whether sequential and geographical influence can be effectively captured by the corresponding models is not guaranteed, since they impose no explicit supervision on the learned user preference. 
%It is worth emphasizing that sequential influence and geographical influence are \textbf{mutual-reinforcing}. Every interaction results from the joint dynamics of sequential and geographical influences. This interaction would, in turn, alter the interaction sequence itself, as well as POI representations nearby. 

% Moreover, sequential and geographical influences have already been entangled with each other in both user-POI interactions and geographical layout of POIs. In most cases, sequential and geographical factors work together in determining where to visit. Nevertheless, the importance of two kinds of influence varies on different user-item interactions. Unfortunately, there is usually no annotated label for the exact importance of these influences in each case, so there is no telling which influence plays the dominant role in an observed interaction. Meanwhile, although the two influences need to be jointly depicted and utilized, traditional models can get confused when the representation of the two influences are entangled. After all, the two influences work in inherently different ways: sequential influence reflects the user's preferences and habits, while geographical influence indicates vicinity and regional traits. Thus, the mixing effect mentioned above may prevent the model from learning high-quality representations of the two influences, hindering its ability to fully utilize both sides of information.

The key to solving this problem is user preference \textbf{disentanglement}, rather than mere combination. Specifically, to depict user preference at a finer granularity and enhance POI recommendation quality, we need to disentangle the two latent driving forces, and thus distill the representations for both influence. The disentanglement of the two influences provides better interoperability, and alleviates the cold-start problem when either of the two influences happens to be sparse. Existing disentanglement models for recommendation either uses dynamic routing (e.g. DGCF \cite{wang2020disentangled}, DisenCTR \cite{wang2022disenctr}) or self-supervised signals (e.g. MacridVAE \cite{ma2019learning}, CLSR \cite{zheng2022disentangling}) to disentangle latent interests, yet how to generate self-supervised signals that disentangle sequential and geographical influences had remained unexplored. 

In a nutshell, the ubiquity and uniqueness of the two influences in LBSNs has poses two major challenges to POI recommendation: \textbf{First.} \textit{How to \textbf{depict} theses two high-order connectivity influences for the user check in data?} \textbf{Second.} \textit{How to explicit \textbf{disentangle} these two influences for POI recommendation?}
%has poses two major challenges to POI recommendation:
%\textbf{First}, how to jointly utilize sequential and geographical relationships as equal counterparts, yet with different propagation schemes along them respectively?
%\textbf{Second}, how to distill disentangled representations for both sequential influence and geographical influence?

To address the aforementioned challenge, we propose \textbf{DisenPOI}, a novel \textbf{Disen}tangled Dual-Graph Framework for \textbf{POI} Recommendation, which explicitly models sequential and geographical influences on user check in data. DisenPOI constructs two disentangled POI graphs: a geographical graph based on spatial affinity, and a sequential graph based on interaction history. To better capture high-order connectivity on different graph topology, two distance- and sequence-aware GNNs are proposed to propagate on the corresponding geographical and  sequential graph. We adopt contrastive learning methods to disentangle the graph representations in a self-supervised way. While there are no ground truth label for the two representations, we obtain their proxies via readout functions on graph to introduce self-supervised signals. With the help of disentangled representations, DisenPOI is able to make recommendations that reflect both sequential and geographical influence.
% To address the aforementioned challenge, we propose \textbf{DisenPOI}, a novel \textbf{Disen}tangled Dual-Graph Framework for \textbf{POI} Recommendation, which explicitly models sequential and geographical influences on user check in data. Specifically, we construct two disentangled graphs using different interactions: a geographical graph based on spatial affinity, and a sequential graph based on interaction history. Then we use a distance-aware GNN to propagate on the geographical graph, and a sequence-aware Gated GNN on the sequential graph. We obtain proxies for both geographical and sequential embeddings as self-supervised signals, disentangling the POI representations acquired from the two graphs for the.
% formulate POI recommendation as a Click-Through Rate (CTR) prediction problem and

%Graph neural networks (GNNs) are suitable for modeling the high-level connectivity on the two graphs. Prevalent GNN recommenders are either CF-based ~\cite{wang2019neural, he2020lightgcn} or sequence-based ~\cite{wu2019session}. Yet, neither of the two paradigms can adequately incorporate location relationship and model geographical influences. We overcome this issue by. 
Our main contributions can be summarized as follows:
\begin{itemize}[leftmargin=*]
\item We construct dual graphs from different interactions to jointly utilize sequential and geographical relationships, devising sequence- and geo-aware propagation schemes for the two graphs respectively to improve embedding quality.
\item We propose to extract disentangled representations of sequential and geographical influences. Sequential and geographical proxies are obtained as self-supervised signals, which are specially tailored for the LBSN setting. To the best of our knowledge, this is the first graph-based POI recommendation framework with disentangled sequential and geographical representations.
\item We conduct extensive experiments on three real-world benchmarks for POI recommendation. Our model consistently outperforms strong baselines, achieving state-of-the-art performance on all three benchmark datasets. We conduct ablation studies to confirm the potency of self-supervised disentanglement to improve POI recommendation quality. We also perform case studies on a selected user, which shows that our disentangled model can generate distinct geographical patterns. 
\end{itemize}

